Data-driven memory-dependent abstractions of dynamical systems

We propose a sample-based, sequential method to abstract a (potentially black-box) dynamical system with a sequence of memory-dependent Markov chains of increasing size. We show that this approximation allows to alleviating a correlation bias that has been observed in sample-based abstractions. We further propose a methodology to detect on the fly the memory length resulting in an abstraction with sufficient accuracy. We prove that under reasonable assumptions, the method converges to a sound abstraction in some precise sense, and we showcase it on two case studies.

==> Sections/Notation.tex <==
\section{Notation}
\label{sec:notation}

Just trying to organise a bit the mathematical notation. Below is a list of main symbols used in our draft:

% All commands are defined in the commands.tex file within the Ancillary folder

\begin{itemize}
    \item We need to have a notation for our alphabet and its monoid that it freely generated by it. My suggestion is to use $\Alphabet$ and $\StarAlphabet$, respectively.
    \item Elements in $\StarAlphabet$ can be denoted by $x$ and $y$, as Raphael suggested in Definition \ref{def-cantorDistance}. Individual entro
    \item Letters $m$, $n$ will denote sizes of elements of $\StarAlphabet$.
    \item The letter $d$ is reserved for the Cantor distance \raphael{about this, it seems that 'cantor' distance is not really standard; apologies. (it seems that Cantor space is standard, but this is slightly more general I think)}
    \licio{We will fix this.}, as in Definition \ref{def-cantorDistance}.
    \item The greek letter $\System$ is reserved to denote a dynamical system. Its behavior will be denoted by $\SysBehavior$.

    %\adrien{There is a conflict with the Borel $\sigma$-algebra $\mathcal{B}(\mathbb{R}^n)$}
    %\licio{This is indeed true. Let's keep this in mind and fix afterwords. One option, which I do not know if you like, is that of overlapping the $\mathcal{B}$ symbol. When it takes an Euclidean space as argument we see it as a $\sigma$-algebra and when its argument is a system $\System$ we see it as the behaviour of the dynamical system $\System$. Not sure if this would be the best option, though...}

    \item Let $B_X$ be the Borel $\sigma$-algebra of $X$. For example it is $B_{\mathbb{R}^n}$ for the euclidian space $\mathbb{R}^n$.
    \adrien{I found this notation in some slides on Internet, I think it is OK. Otherwise we just not mention it as Raphaël suggested.}
    \licio{Great! I am happy with it, although we may not refer to Borel $\sigma$-algebras in later versions.}
    \item $\OutputMap$ is the output of the dynamical system and $\MemoryOutput{\ell}$ (with subscript) the output of the memory-$\ell$ Markov model.
    \item The symbol $\ell$ is being employed to refer to the $\ell$-complete setting.
    \item $\mathbb{N}$ is the set of natural numbers
    \item $\mathbb{Q}_k$, for some natural number $k$, is the measurable induced by our dynamical system 
    \item I am using $i$ to represent an infinite sequence of switching signals
    \item $\samplings_{x}$ represents the number of samplings where we have observed $x$
    \item $\delta_{A}$ is the Dirac measure for the set $A$, it is defined as 
    \[ 
        \delta_A(x) = \begin{cases}
            1 \quad \text{if } x \in A, \\
            0 \quad \text{otherwise.}
        \end{cases}
    \]
    
\end{itemize}
